Schema Independent Relational Learning

Learning novel concepts and relations from relational databases is an important problem with many applications in database systems and machine learning. Relational learning algorithms learn the definition of a new relation in terms of existing relations in the database. Nevertheless, the same data set may be represented under different schemas for various reasons, such as efficiency, data quality, and usability. Unfortunately, the output of current relational learning algorithms tends to vary quite substantially over the choice of schema, both in terms of learning accuracy and efficiency. This variation complicates their off-the-shelf application. In this paper, we introduce and formalize the property of schema independence of relational learning algorithms, and study both the theoretical and empirical dependence of existing algorithms on the common class of (de) composition schema transformations. We study both sample-based learning algorithms, which learn from sets of labeled examples, and query-based algorithms, which learn by asking queries to an oracle. We prove that current relational learning algorithms are generally not schema independent. For query-based learning algorithms we show that the (de) composition transformations influence their query complexity. We propose Castor, a sample-based relational learning algorithm that achieves schema independence by leveraging data dependencies. We support the theoretical results with an empirical study that demonstrates the schema dependence/independence of several algorithms on existing benchmark and real-world datasets under (de) compositions.

==> EmpiricalBeyondComposition.tex <==

%\subsection{Beyond Decomposition and Composition}
%\label{section:experiments-beyond}
\begin{table}%[!htbp]
	\begin{center}
		{\scriptsize
			\centering
			\begin{tabular} {c|c|c|c|c}
				\hline
				\multicolumn{5}{c}{HIV-2K4K} \\
				\hline			
				Metric & Initial & \multicolumn{2}{c|}{4NF-1} & 4NF-2  \\
				\hline
				Precision	& 0.77	& \multicolumn{2}{c|}{0.79} & 0.73 	\\
				Recall	& 0.63	& \multicolumn{2}{c|}{0.87} & 0.76 	\\
				Time (min)	& 27	&  \multicolumn{2}{c|}{14.8} & 576 \\
				
				\hline
				\multicolumn{5}{c}{UW-CSE} \\
				\hline			
				Metric & Original & 4NF & Denorm-1 & Denorm-2  \\
				\hline
				Precision	& 0.93	& 0.93 & 0.93 & 0.93	\\
				Recall	& 0.54	& 0.54 & 0.54	& 0.54	\\
				Time (s)	& 8	&  8.9 & 9.1	& 13.3 \\
				
				\hline
				\multicolumn{5}{c}{IMDb} \\
				\hline			
				Metric & JMDB & \multicolumn{2}{c|}{Stanford} & Denormalized  \\
				\hline
				Precision	& 1	& \multicolumn{2}{c|}{0.98} & 1 	\\
				Recall	& 1	& \multicolumn{2}{c|}{0.84} & 1 	\\
				Time (min)	& 7.3	&  \multicolumn{2}{c|}{90.8} & 8.1	 \\
			\end{tabular}}
%			\vspace{-6pt}
			\caption{{\small Results of Castor learning relations over HIV-2K4K, UW-CSE and IMDb data using only INDs in the form of subset.}}
			\label{table:beyondcomposition}
%			\vspace{-13pt}
		\end{center}
	\end{table}

\noindent
{\bf General decomposition/ composition.}
%We focus on transformations where the target schema contains only INDs in the form of subset, defined as foreign key (FK) to primary key (PK) constraints. 
To explore non-bijective decomposition/ compositions of 
HIV, UW-CSE, and IMDb, we restore the INDs with equality that we have enforced on their schemas to their original forms. 
%TODO: mention the original form of INDs with equality in IMDb.
For instance, we restore the enforced INDs with equality {\it movies2X[id] = movie[id]} in IMDb schemas to \\ 
{\it movies2X[id] $\subseteq$ movie[id]} in IMDb schemas. 
We also modify the INDs with equality that are originally found in these datasets to INDs in form of foreign key 
to primary key referential integrities in their schemas. 
For example, we have changed INDs {\it movies2X[Xid] = X[id]} to {\it movies2X[Xid] $\subseteq$ X[id]} over IMDb schemas. 
Hence, the transformations explained in Section~\ref{section:empirical-settings} for these datasets are 
general decomposition/ composition and not bijective. 
We run the extended version of Castor from Section~\ref{sec:generalDecomposition} using the aforementioned INDs and all other regular INDs in each schema.
The extension of Castor gets the same results as in Table~\ref{tableuwcseres67} 
over UW-CSE and is schema independent. It is also robust and
delivers the same results as in Table~\ref{tableimdbres67} for JMDB and Denormalized schemas 
of IMDb. But, it returns precision of 0.98 and recall of 0.84 over the database with 
Stanford schema. Overall, it is more effective and schema independent than other algorithms over IMDb.
%Over these datasets, this extension of Castor first encounters and selects tuples from relations on the left hand of INDs, e.g., relations that contain foreign keys, in bottom-clause construction. Thus, it selects tuples from relations on the right hand side of INDs and create equivalent bottom-clauses across schemas. 
However, the results of the extension of Castor vary with the schema over the HIV-2K4K dataset: it delivers precision of 
0.77,  0.79, and 0.73 and recall of 0.63, 
0.87, and 0.76 over the Initial, 4NF-1, and 4NF-2 schemas, respectively. 
This is because it cannot access some tuples in the bottom-clause construction in these databases as explained in Section~\ref{sec:generalDecomposition}. 
Its precisions are equal or higher than the those of Aleph-FOIL and Aleph-Progol over all schemas and its recall is higher than that of Aleph-FOIL and Aleph-Progol in 4NF-2 schema.
But, its recall is lower than the recall of Aleph-FOIL and Aleph-Progol over the Initial and Aleph-Progol over 4NF-1 schemas.
Table~\ref{table:beyondcomposition} shows the results of Castor learning relations over the HIV-2K4K, UW-CSE and IMDb datasets, using only INDs in the form of subset.
For HIV-2K4K, it uses the INDs in Table~\ref{table:hiv-INDs} (bottom).
For UW-CSE, it uses the INDs in Table~\ref{table:uwcse-INDs} (bottom).
For IMDb, it uses the INDs in Table~\ref{table:imdb-INDs} (bottom).



\begin{comment}
We use the FK to PK constraints shown as INDs in the form of subset in Tables~\ref{table:hiv-INDs}, \ref{table:uwcse-INDs} and \ref{table:imdb-INDs} (bottom) in Appendix~\ref{appendix:schemas}.
Table~\ref{table:beyondcomposition} in Appendix~\ref{appendix:discussion} shows the results.
Castor is successful over UW-CSE and IMDb for two reasons: 
1) Castor follows a bottom-up search approach, which is less affected by heuristics. This is also reflected in the results achieved by ProGolem in UW-CSE, which is nearly robust.
2) In bottom-clause construction, Castor accesses relations that are in a FK. Then, Castor can also access relations on the right hand side of the FK to PK constraint.
For instance, in the UW-CSE dataset, given tuple {\it taughtBy(c,p,t)}, Castor can access tuple {\it courseLevel(c,l)}.
In the IMDb dataset, given tuple {\it movies2genres(m,g)}, Castor can access tuple {\it genre(g,drama)}.
Without using INDs, other algorithms are not be able to access these tuples, unless parameters are modified.
\end{comment}


\begin{comment}
For this experiment we use the UW-CSE dataset, as it is the only one for which all algorithms scale.
%Therefore, we are able to evaluate and compare the schema independence of all algorithms.
We use the FK to PK constraints shown in Table~\ref{table:uwcse-INDs} (bottom) in Appendix~\ref{appendix:schemas}.
%We define the following FK to PK constraints: 
%{\it hasPosition[prof] $\subseteq$ professor[prof]}, 
%{\it inPhase[stud] $\subseteq$ student[stud]}, 
%{\it yearsInProgram[stud] $\subseteq$ student[stud]}, 
%{\it taughtby[prof] $\subseteq$ professor[prof]}, and
%{\it taughtby[crs] $\subseteq$ courseLevel[crs]}.
%The results of Castor using only FK to PK constraints are shown in Table~\ref{tableuwcse-onewayINDs}. 
Even with INDs in the form of subset, Castor gets the same results shown in Table~\ref{tableuwcseres67}.
This happens for two reasons: 
1) Castor follows a bottom-up search approach, which is less affected by heuristics. This is also reflected in the results achieved by ProGolem, which is nearly robust.
2) In bottom-clause construction, Castor accesses relations that have a FK. Then, Castor can also access relations on the right hand side of the FK to PK constraint.
For instance, given tuple {\it taughtBy(c,p,t)}, Castor can access tuple {\it courseLevel(c,l)}.
Without using INDs, an algorithm would not be able to access this tuple, unless parameters are modified.
%The argument given in point 2 does not happen in every dataset, which may cause Castor to not be completely schema independent.
%Therefore, as future work, we will try to modify Castor so that it is schema independent over this and other types of transformations.
\end{comment}

%Castor is not schema independent, as there are slight variations in its precision and recall scores along different schemas. 
%However, it is still relatively robust.
%It is also more robust than other algorithms.
%The reason is that Castor exploits data dependencies that are commonly present in relational schemas. 
%On the other hand, other algorithms do not leverage this information.
%As future work, we will try to modify Castor so that it is schema independent on this and other types of transformations.

%\begin{table}[t]%[!htbp]
%	\begin{center}
%		{\scriptsize
%			\centering
%			%P{0.13\columnwidth} | P{0.13\columnwidth} | P{0.10\columnwidth} | P{0.10\columnwidth}
%			\begin{tabular} { c | c | c | c | c | c }
%				\hline
%				Algorithm & Metric & Original & 4NF & Denorm-1 & Denorm-2  \\
%				\hline			
%				\multirow{3}{*}{Castor} & Precision	& 0.931 & 0.929 & 0.929 & 0.929 \\
%				& Recall	& 0.542 	& 0.536	& 0.536 & 0.536 \\
%				& Time (s)	& 8 & 8.9 & 9.1 & 13.3 \\
%			\end{tabular}}
%			\vspace{-6pt}
%			\caption{{\small Results of learning relations over UW-CSE data.}}
%			\label{tableuwcse-onewayINDs}
%			\vspace{-13pt}
%		\end{center}
%	\end{table}


%



==> SchemaIndependence.tex <==
\subsection{Schema independence of learning algorithms}
\label{schema_independence}


Relational learning algorithms can be viewed as a search problem for a hypothesis that deduces the training data, following either a top-down or bottom-up approach.
Top-down algorithms~\cite{Quinlan:FOIL, progol} start from the most general hypothesis and employ specialization operators to get more specific hypotheses. A common specialization operator is the addition of a new literal to the body of a clause. 
On the other hand, bottom-up algorithms~\cite{golem, progolem, MuggletonBu88} start from specific hypotheses that are constructed based on the training examples, and use generalization operators to search the hypothesis space. Generalization operators include inverse resolution, relative least general generalization, asymmetric relative minimal generalization, among others.
Therefore, a generic relational learning algorithm can be seen as a sequence of steps, where in each step an operator is applied to the current hypothesis. 

Let $RLA$ (Relational Learning Algorithm) be an algorithm that takes as input training data $E$, background knowledge $B$, and target relation $T$, and learns a hypothesis $H$ that, together with $B$, entails $E$. This type of learning algorithms is studied by the field of Inductive Logic Programming (ILP).
\begin{definition}
	Given background knowledge $B$, positive examples $E^+$, negative examples $E^-$, and a target relation $T$, the ILP task is to find a definition $H$ for $T$ such that:
	\begin{itemize}
		\item $\forall p \in E^+, H \wedge B \models p$ (completeness)
		\item $\forall p \in E^-, H \wedge B \not\models p$ (consistency)
	\end{itemize}
\end{definition}
$E$, $H$ and $B$ are each logic programs. $E$ usually contains ground unit clauses of a single target predicate $T$, which express positive ($E^+$) or negative ($E^-$) examples. $H$ is usually restricted to Horn definitions for efficiency reasons. $B$ can contain arbitrary logic programs. In this paper, we focus in extensional background knowledge, which consists of ground atoms, and can be expressed in the form of a database instance.

Consider FOIL~\cite{Quinlan:FOIL}, a greedy, top-down relational learning algorithm. FOIL follows a covering approach that consists of two loops: an outer loop that constructs a clause one at a time, and an inner loop that iteratively specializes the clause being constructed. The inner loop starts with the most general clause, which is the empty clause, and specializes it by adding literals, until a stopping criterion is met (consistency). After building a clause, the algorithm adds the clause to the hypothesis, discards the positive examples covered by the clause, and tries to learn a new clause. The algorithm exits from the outer loop when all positive examples have been covered (completeness), and the resulting hypothesis is the Horn definition for the target relation.

\begin{example}
	\label{example:relational_learning}
	Consider using FOIL and the UW-CSE database to learn a definition for the target relation {\it collaborated(X,Y)}, which indicates that person $X$ has collaborated with person $Y$. The inner loop in FOIL starts with the empty clause $collaborated(X,Y) \leftarrow .$, which covers all positive and negative examples. After some iterations, the constructed clause is
	\begin{eqnarray*}
	collaborated(X,Y) \leftarrow project(P,X), project(P,Y).
	\end{eqnarray*}
	This clause satisfies the stopping criterion, so FOIL exists from the inner loop.
	The clause also covers all positive examples in the training data, so the algorithm exits from the outer loop, having successfully learned a definition for the target relation.
\end{example}

Usually, the hypothesis space of relational learning algorithms is very big, requiring a lot of resources (e.g. time and space). In practice, the amount of resources used by these algorithms must be restricted by some parameter settings.
%For instance, we may restrict the number of times that a specialization or generalization operator is applied. 
These parameter settings are common in ILP systems that implement relational learning algorithms. 
Let the {\it parameter settings} be a tuple of variables $\langle p_1, ..., p_r \rangle$, where each  parameter $p_i$ sets an upper bound on a variable that restricts the use of some computational resource, directly or indirectly. 
%imposes a restriction on some resource directly or indirectly. 
In this paper we assume that each parameter $p_i$ is of a generic type.
%, and that $p_i \ge n_0$, where $n_0$ is the minimum number so that the algorithm is able to learn equivalent definitions over different schemas. 
%The set of all possible parameter settings, that is all possible combinations of values for all different parameters, is the {\it parameter space}. 
We say that an algorithm is {\it bounded} if it is restricted by some parameter settings. To get theoretical insights, we also analyze the {\it unbounded} versions of learning algorithms, which have empty parameters.

For instance, top-down algorithms perform search on a graph, where each node in the graph is a clause. A new literal is added to a clause in every specialization step, and this is represented by a new node in the graph.
The space of candidate literals for a predicate is $O(k^a)$, where $k$ is the number of variables in the clause and $a$ is the arity of the predicate. The branching factor for each node, that is the number of children of the node, is $O(pk^a)$, where $p$ is the number of different relations in the schema. 
Therefore, the number of nodes in the graph is $O((pk^a)^d)$, where $d$ is maximum depth of the graph (tree).
A parameter may be the maximum number of nodes $n$ such that $O((pk^a)^d) \le n$, or the maximum depth $l$ such that the number of nodes is bounded by $O((pk^a)^l)$.

% PARAMETER SETTINGS MAPPING FUNCTION
\begin{comment}
A {\it mapping} of parameter settings is an invertible, total function $f\colon \mathbb{P} \to \mathbb{P}$, where $\mathbb{P}$ is the parameter space. One mapping function $f$ is defined for a source and target schema, so that it takes as input some parameter settings for the source schema and returns the equivalent parameter settings for the target schema.
The function $f$ must be total, as there must be a mapping for every parameter setting in the source schema to the target schema.
\end{comment}

There is a trade-off between computational resources used by an algorithm and the size of its hypothesis space. 
Parameter settings are set so that an algorithm can be used in practice, with the hope that the algorithm will find a consistent and complete hypothesis.
\begin{example}
	\label{example:parameter_settings}
	Continuing Example~\ref{example:relational_learning}, consider the parameter clause-length, which sets an upper bound on the numbers of literals in a learned clause (including the head literal). 
	Assume that we are now interested in learning a definition for the target relation {\it collaboratedProf(X,Y)}, which indicates that professor $X$ has collaborated with professor $Y$, under the original schema. 
	If we set clause-length $= 5$, FOIL is able to learn the complete and consistent definition
	\begin{align*}
		collaboratedProf(X,Y) &\leftarrow professor(X), professor(Y), \\
		& project(P,X), project(P,Y).
	\end{align*}
	However, if we set clause-length $= 3$, FOIL is not able to learn this definition as its length is 5. With clause-length $= 3$, FOIL is not able to learn a complete and consistent definition for the target relation {\it collaboratedProf(X,Y)}.
\end{example}
	

%$RLA$ is {\it schema independent} if, by taking the same background information expressed under different schemas, it can learn equivalent Horn definitions for the target relation given some parameter settings.

%\begin{definition}
%	\label{schema_independence}
%	Let $\mR$ and $\mS$ be two definition equivalent schemas that are able to express the same background information $B$. 
%	Let $H_{\mR}$ and $H_{\mS}$ be the Horn definitions learned by $RLA$ for any target relation $T$ under $\mR$ and $\mS$ with parameter settings ${\bf p_{\mR}}$ and ${\bf p_{\mS}}$, respectively. 
%	$RLA$ is schema independent if and only if $H_{\mR}$ and $H_{\mS}$ are equivalent.
%\end{definition}

We now define the notion of schema independence for relational learning algorithms.
\begin{definition}
	\label{schema_independence}
	Let $\mR$ and $\mS$ be two definition equivalent schemas, and $I$ and $J$ be database instances of $\mR$ and $\mS$, respectively, so that instance $J$ is the result of a transformation of instance $I$.
	%Let $f$ be the function that maps parameters settings in $\mR$ to parameter settings in $\mS$.
	Let $H_{\mR}$ be the Horn definition learned by $RLA$ for some target relation $T$ with training data $E$, input $I$, and parameter settings ${\bf p}$.
	$RLA$ is schema independent if and only if:
	\begin{itemize}
		\item $RLA$ learns Horn definition $H_{\mS}$ for target relation $T$ with training data $E$, input $J$, and same parameter settings ${\bf p}$; and
		\item $H_{\mR}$ and $H_{\mS}$ are equivalent.
	\end{itemize}
\end{definition}
% PARAMETER SETTINGS MAPPING FUNCTION
\begin{comment}
\begin{definition}
	\label{schema_independence}
	Let $\mR$ and $\mS$ be two definition equivalent schemas, and $I$ and $J$ be database instances of $\mR$ and $\mS$, respectively, so that instance $J$ is the result of a vertical transformation of instance $I$.
	Let $f$ be the function that maps parameters settings in $\mR$ to parameter settings in $\mS$.
	Let $H_{\mR}$ be the Horn definition learned by $RLA$ for some target relation $T$ with training data $E$, input $I$, and parameter settings ${\bf p_{\mR}}$.
	$RLA$ is schema independent if and only if:
	\begin{itemize}
		\item $f({\bf p_{\mR}}) = {\bf p_{\mS}}$ such that $RLA$ learns Horn definition $H_{\mS}$ for target relation $T$ with training data $E$, input $J$, and parameter settings ${\bf p_{\mS}}$; and
		\item $H_{\mR}$ and $H_{\mS}$ are equivalent.
	\end{itemize}
\end{definition}
\end{comment}
Notice that $RLA$ takes the exact same training data $E$, as well as equivalent database instances $I$ and $J$.
In this paper, we only consider vertical transformations of database instances. Therefore, when we say that an algorithm is (not) schema independent, we mean that it is (not) schema independent under vertical transformations.

\begin{example}
	\label{example:schema_independence}
	Consider the original schema and schema 4 in Table~\ref{table:uwcse}. The original schema is the result of a vertical decomposition of schema 4.
	If the target relation is {\it collaboratedProf(X,Y)}, as in Example~\ref{example:parameter_settings}, FOIL is able to learn equivalent definitions under the original schema and schema 4.
	However, if the target relation is {\it advisedBy(X,Y)}, FOIL learns non-equivalent definitions under these schemas. Under the original schema, it learns a definition based on co-authorship:
	\begin{align*}
		advisedBy(X,Y) &\leftarrow student(X), professor(Y), \\
		& publication(P,X), publication(P,Y).
	\end{align*}
	On the other hand, under schema 4, FOIL learns a definition based on courses taught by the professor in which the student has been TA:
	\begin{eqnarray*}
		advisedBy(X,Y) \leftarrow course(C,Y,X,T,L).
	\end{eqnarray*}
	Therefore, FOIL is not schema independent.
\end{example}
In the following sections we analyze the schema independence of stand-alone learning algorithms, as well as algorithms that implement specialization and generalization operators.



% DIFFERENT NOTIONS OF SCHEMA INDEPENDENCE

\begin{comment}

We now define different degrees of schema independence that are based on the parameter settings imposed to the algorithms that implement these operators, as well as the output produced by the algorithms. 

$RLA$ is {\it weakly schema independent} if, by taking the same background information expressed under different schemas, it can learn equivalent Horn definitions for the target relation, without regard of the parameter settings.


\begin{definition}
	\label{weak_schema_independence}
	Let $\mR$ and $\mS$ be two definition equivalent schemas that are able to express the same background information $B$. 
	Let $H_{\mR}$ and $H_{\mS}$ be the Horn definitions learned by $RLA$ for any target relation $T$ under $\mR$ and $\mS$, respectively. 
	$RLA$ is {\bf weakly schema independent} if and only if $H_{\mR}$ and $H_{\mS}$ are equivalent.
	%$RLA$ is weakly schema independent if and only if it can learn equivalent Horn definitions $H_{\mR}$ and $H_{\mS}$, under $R$ and $S$, respectively. 
\end{definition}


Definition \ref{weak_schema_independence} gives a weak notion of schema independence, where it is only required that the algorithm learns equivalent clauses, but there is no restriction on the amount of resources used by the algorithm.
However, in order to use this algorithm in practice, resources should be restricted by setting some parameters.
For instance, we may restrict the number of times that a specialization or generalization operator is applied. 
These parameter settings are common in ILP systems that implement relational learning algorithms. 
For this reason, we define a stronger notion of schema independence that takes this into consideration.

%\begin{definition}
%\label{strong_schema_independence}
%Let ${\bf C_{\mR}}$ be the set of clauses learned with at most $l$ steps under schema $\mR$.
%, and ${\bf C_{\mS}}$ be the set of clauses learned with at most $l'$ steps under schema $\mS$.
%$RLA$ is strongly schema independent if and only if for every target relation $T$ and the set of clauses ${\bf C_{\mR}}$, there is a number $l'$ such that all clauses equivalent to clauses in ${\bf C_{\mR}}$ can be learned with $l'$ steps under schema $\mS$, and no more clauses are learned.
%\end{definition}


\begin{definition}
	\label{strong_schema_independence}
	Let $\mR$ and $\mS$ be two definition equivalent schemas that are able to express the same background information $B$. 
	Let $H_{\mR}$ be the Horn definition learned by $RLA$ for any target relation $T$ under $\mR$ with parameter settings ${\bf p_{\mR}}$.
	$RLA$ is {\bf strongly schema independent} if and only if:
	\begin{itemize}
		\item There exists an invertible mapping function $f(\mR, \mS, {\bf p_{\mR}}) = {\bf p_{\mS}}$ so that $RLA$ is able to learn Horn definition $H_{\mS}$ for target relation $T$ under $\mS$ with parameter settings ${\bf p_{\mS}}$; and
		\item $H_{\mR}$ and $H_{\mS}$ are equivalent.
	\end{itemize}
	%Let $T$ be the target relation, $S$ and $R$ two definition equivalent schemas. and $C$ be an arbitrary Horn definition learned in $l$ steps, under schema $\mS$. $RLA$ is strongly schema independent if and only if an invertible function $f: N \to N$  exists such that $f(l) = l'$, when $l'$ is the number of steps needed to learn the Horn definition $C'$ under schema $\mR$, which is equivalent to $C$. 
\end{definition}

\begin{definition}
	\label{strong_schema_independence}
	(ALTERNATIVE DEFINITION) Let $\mR$ and $\mS$ be two definition equivalent schemas that are able to express the same background information $B$. 
	Let ${\bf H_{\mR}}$ be the set of all Horn definitions that can be learned by $RLA$ for all target relations under $\mR$ with parameter settings ${\bf p_{\mR}}$.
	$RLA$ is {\bf strongly schema independent} if and only if:
	\begin{itemize}
		\item There exists an invertible mapping function $f(\mR, \mS, {\bf p_{\mR}}) = {\bf p_{\mS}}$ so that ${\bf H_{\mS}}$ is the set of all Horn definitions that can be learned by $RLA$ for all target relations under $\mS$ with parameter settings ${\bf p_{\mS}}$; and
		\item ${\bf H_{\mR}}$ and ${\bf H_{\mS}}$ are bijective sets where every Horn definition $H_{\mR} \in {\bf H_{\mR}}$ is equivalent with its correspondent Horn definition $H_{\mS} \in {\bf H_{\mS}}$.
	\end{itemize}
\end{definition}


An algorithm that is {\it strongly schema independent} is useful in practice because it can be tuned to get the same results under equivalent schemas. That is, after tuning the algorithm to work under the source schema, it can be tuned again to work under the destination schema, and both will produce the same results. 

KEEP THIS? There is an even stronger condition for schema independence, where the algorithm is required to take exactly the same number of steps to learn equivalent sets of clauses under different schemas. This condition makes an ideal scenario where an algorithm has to be tuned only once and can be used with different schemas and get the same results. However this condition is too strong and can be easily rejected with the following example: ADD EXAMPLE TO REJECT THIS CONDITION.
%\begin{example}
%Consider schemas $\mR$ and $\mS$ shown in Table~\ref{example_schemas}, and target clauses $C_{\mR} = E(X,Y) \leftarrow P(X,Z) \wedge Q(Z,Y)$ and $C_{\mS} = E(X,Y) \leftarrow R(X,Z,Y)$, as shown in Example~\ref{inverse_resolution_example1}. Algorithm $RLA$ requires $l=2$ steps to learn clause $C_{\mR}$, however it only requires $l'=1$ step to learn clause $C_{\mS}$. There are no numbers $l$ and $l'$ such that $l = l'$ and $IIR$ is able to learn equivalent clauses under both schemas.
%\end{example}
%
%\begin{table}[h]
%\centering
%\begin{tabular} {| p{0.5\linewidth} | p{0.5\linewidth} |}
%\hline
%Schema $\mR$ & Schema $\mS$ \\
%\hline
%$P(A_1,A_2)$ & $R(A_1,A_2,A_3)$ \\
%$Q(A_1,A_2)$ &  \\
%\hline
%$E(A_1,A_2)$ & $E(A_1,A_2)$ \\
%\hline
%$\Sigma = \{P.A_1 \rightarrow P.A_2; Q.A_1 \rightarrow Q.A_2\}$ & $\Omega = \{R.A_1 \rightarrow R.A_2,R.A_3\}$ \\
%\hline
%\end{tabular}
%\caption{Two equivalent schemas, $\mS$ is a vertical transformation of $\mR$.  }
%\label{example_schemas}
%\end{table}

\end{comment}

